Fast simulation of light scattering and harmonic generation in axially symmetric structures in COMSOL

In the field of optics and nanophotonics, simulation of electromagnetic scattering plays a major role in the study of complex nanostructures and optical devices. The numerical analysis of scattering spectra, even for nanocavities with simple geometry, is associated with significant computational difficulties. However, when the system exhibits certain symmetries, it becomes possible to simplify the problem through the process of separation of variables, which leads to a decrease in its dimension. In this paper, we aim to provide a practical guide to a fast simulation of linear and non-linear scattering problems in COMSOL Multiphysics for axisymmetric objects including computation of scattering cross-section as well as its multipolar decomposition, optical forces, and second harmonic generation. We also accompany the provided guide with the ready-to-run COMSOL models.

==> sections/code.tex <==


\begin{lstlisting}[language=Mathematica,caption={Electric multipoles}, numbers=none]

ClearAll;


CON = -k1^2/Sqrt[8Pi]*1/(Sqrt[(2Pi)^3]/8/Pi^2);

Yjmconj0 = 1/2/Sqrt[Pi];

conjY11 = Exp[-2*I*\[Phi]]*SphericalHarmonicY[1,1,\[Theta],\[Phi]];
conjY10 =SphericalHarmonicY[1,0,\[Theta],\[Phi]];
conjY1m1 = Exp[2*I*\[Phi]]*SphericalHarmonicY[1,-1,\[Theta],\[Phi]];
Yjmconj1 = {conjY11, conjY10,conjY1m1};

conjY2m2 =Exp[4*I*\[Phi]]*SphericalHarmonicY[2,-2,\[Theta],\[Phi]];
conjY2m1=Exp[2*I*\[Phi]]*SphericalHarmonicY[2,-1,\[Theta],\[Phi]] ;
conjY20=SphericalHarmonicY[2,0,\[Theta],\[Phi]];
conjY21 =Exp[-2*I*\[Phi]]*SphericalHarmonicY[2,1,\[Theta],\[Phi]];
conjY22 =Exp[-4*I*\[Phi]]*SphericalHarmonicY[2,2,\[Theta],\[Phi]];

Yjmconj2 ={conjY22,conjY21,conjY20,conjY2m1,conjY2m2};

conjY33 =Exp[-6*I*\[Phi]]*SphericalHarmonicY[3,3,\[Theta],\[Phi]];
conjY32 =Exp[-4*I*\[Phi]]*SphericalHarmonicY[3,2,\[Theta],\[Phi]];
conjY31 =Exp[-2*I*\[Phi]]*SphericalHarmonicY[3,1,\[Theta],\[Phi]];
conjY30 = SphericalHarmonicY[3,0,\[Theta],\[Phi]];
conjY3m1 =Exp[2*I*\[Phi]]*SphericalHarmonicY[3,-1,\[Theta],\[Phi]];
conjY3m2 = Exp[4*I*\[Phi]]*SphericalHarmonicY[3,-2,\[Theta],\[Phi]];
conjY3m3 =Exp[6*I*\[Phi]]*SphericalHarmonicY[3,-3,\[Theta],\[Phi]];

Yjmconj3 ={conjY33, conjY32,conjY31,conjY30,conjY3m1,conjY3m2, conjY3m3};

conjY44 = Exp[-8*I*\[Phi]]*SphericalHarmonicY[4,4,\[Theta],\[Phi]];
conjY43 =Exp[-6*I*\[Phi]]*SphericalHarmonicY[4,3,\[Theta],\[Phi]];
conjY42 = Exp[-4*I*\[Phi]]*SphericalHarmonicY[4,2,\[Theta],\[Phi]];
conjY41 =Exp[-2*I*\[Phi]]*SphericalHarmonicY[4,1,\[Theta],\[Phi]];
conjY40 =SphericalHarmonicY[4,0,\[Theta],\[Phi]];
conjY4m1 =Exp[2*I*\[Phi]]*SphericalHarmonicY[4,-1,\[Theta],\[Phi]];
conjY4m2 = Exp[4*I*\[Phi]]*SphericalHarmonicY[4,-2,\[Theta],\[Phi]];
conjY4m3 =Exp[6*I*\[Phi]]*SphericalHarmonicY[4,-3,\[Theta],\[Phi]];
conjY4m4 = Exp[8*I*\[Phi]]*SphericalHarmonicY[4,-4,\[Theta],\[Phi]];

Yjmconj4={conjY44,conjY43,conjY42,conjY41,conjY40,conjY4m1,conjY4m2,conjY4m3,conjY4m4} ;

conjY55 = Exp[-10*I*\[Phi]]*SphericalHarmonicY[5,5,\[Theta],\[Phi]];
conjY54 = Exp[-8*I*\[Phi]]*SphericalHarmonicY[5,4,\[Theta],\[Phi]];
conjY53 =Exp[-6*I*\[Phi]]*SphericalHarmonicY[5,3,\[Theta],\[Phi]];
conjY52 = Exp[-4*I*\[Phi]]*SphericalHarmonicY[5,2,\[Theta],\[Phi]];
conjY51 =Exp[-2*I*\[Phi]]*SphericalHarmonicY[5,1,\[Theta],\[Phi]];
conjY50 =SphericalHarmonicY[5,0,\[Theta],\[Phi]];
conjY5m1 =Exp[2*I*\[Phi]]*SphericalHarmonicY[5,-1,\[Theta],\[Phi]];
conjY5m2 = Exp[4*I*\[Phi]]*SphericalHarmonicY[5,-2,\[Theta],\[Phi]];
conjY5m3 =Exp[6*I*\[Phi]]*SphericalHarmonicY[5,-3,\[Theta],\[Phi]];
conjY5m4 = Exp[8*I*\[Phi]]*SphericalHarmonicY[5,-4,\[Theta],\[Phi]];
conjY5m5 = Exp[10*I*\[Phi]]*SphericalHarmonicY[5,-5,\[Theta],\[Phi]];

Yjmconj5={conjY55,conjY54,conjY53,conjY52,conjY51,conjY50,conjY5m1,conjY5m2,conjY5m3,conjY5m4,conjY5m5} ;


J1 = (Cos[\[Phi]] - I *Sin[\[Phi]])/Sqrt[2]*(-Jro+I*Jphi);
J0 = Jz;
Jm1 = (Cos[\[Phi]] + I*Sin[\[Phi]])/Sqrt[2]*(Jro+I*Jphi);

F[mb_]:={J1*Exp[I*mb*\[Phi]],J0*Exp[I*mb*\[Phi]],Jm1*Exp[I*mb*\[Phi]]};


Print[StringForm["Dipole"]]

j = 1;
(*%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%*)

X1[j_,m_]:=-1/(j*(j+1))^(1/2)*((j*(j+1)-m*(m-1))/2)^(1/2)*SphericalHarmonicY[j,m-1,\[Theta],\[Phi]];
X2[j_,m_]:=1/(j*(j+1))^(1/2)*m*SphericalHarmonicY[j,m,\[Theta],\[Phi]];
X3[j_,m_]:=1/(j*(j+1))^(1/2)*((j*(j+1)-m*(m+1))/2)^(1/2)*SphericalHarmonicY[j,m+1,\[Theta],\[Phi]];
For[nn=0,nn<2j+1,nn++,
m=j-nn;





Xjm={X1[j,m],X2[j,m],X3[j,m]} ;
Xjm//MatrixForm;

Z1= I*I*(-SphericalHarmonicY[1,-1,\[Theta],\[Phi]]*X2[j,m]- SphericalHarmonicY[1,0,\[Theta],\[Phi]]*X1[j,m])*2*Sqrt[Pi/3];
Z2= I*I*(-SphericalHarmonicY[1,-1,\[Theta],\[Phi]]*X3[j,m]+SphericalHarmonicY[1,1,\[Theta],\[Phi]]*X1[j,m])*2*Sqrt[Pi/3];
Z3= I*I*(SphericalHarmonicY[1,0,\[Theta],\[Phi]]*X3[j,m]+SphericalHarmonicY[1,1,\[Theta],\[Phi]]*X2[j,m])*2*Sqrt[Pi/3];
Zjm={Z1,Z2,Z3} ;


(*%%%%%%%%%%%%%%%% lb=j-1   %%%%%%%%%%%%%%%%%%%%%%*)
lb=j-1;
aShaddedMinus=Table[Integrate[Conjugate[Zjm]*SphericalHarmonicY[lb,mb,\[Theta],\[Phi]]*Sin[\[Theta]],{\[Theta],0,Pi},{\[Phi],0,2*Pi}].F[m]*j0*CON*(-I)^(lb+j-1),{mb,lb,-lb,-1}];





lb=j+1;
aShaddedMinus1=Table[Integrate[Conjugate[Zjm]*SphericalHarmonicY[lb,mb,\[Theta],\[Phi]]*Sin[\[Theta]],{\[Theta],0,Pi},{\[Phi],0,2*Pi}].F[m]*j2*CON*(-I)^(lb+j-1),{mb,lb,-lb,-1}];



Print[StringForm["m = ``",-m]];

Print[Simplify[Integrate[r*(aShaddedMinus.Yjmconj0 +aShaddedMinus1.Yjmconj2),{\[Phi],0,2*Pi}]]];




]



Print[StringForm["Quadropole"]]

j = 2;
(*%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%*)

X1[j_,m_]:=-1/(j*(j+1))^(1/2)*((j*(j+1)-m*(m-1))/2)^(1/2)*SphericalHarmonicY[j,m-1,\[Theta],\[Phi]];
X2[j_,m_]:=1/(j*(j+1))^(1/2)*m*SphericalHarmonicY[j,m,\[Theta],\[Phi]];
X3[j_,m_]:=1/(j*(j+1))^(1/2)*((j*(j+1)-m*(m+1))/2)^(1/2)*SphericalHarmonicY[j,m+1,\[Theta],\[Phi]];
For[nn=0,nn<2j+1,nn++,
m=j-nn;




Xjm={X1[j,m],X2[j,m],X3[j,m]} ;
Xjm//MatrixForm;

Z1= I*I*(-SphericalHarmonicY[1,-1,\[Theta],\[Phi]]*X2[j,m]- SphericalHarmonicY[1,0,\[Theta],\[Phi]]*X1[j,m])*2*Sqrt[Pi/3];
Z2= I*I*(-SphericalHarmonicY[1,-1,\[Theta],\[Phi]]*X3[j,m]+SphericalHarmonicY[1,1,\[Theta],\[Phi]]*X1[j,m])*2*Sqrt[Pi/3];
Z3= I*I*(SphericalHarmonicY[1,0,\[Theta],\[Phi]]*X3[j,m]+SphericalHarmonicY[1,1,\[Theta],\[Phi]]*X2[j,m])*2*Sqrt[Pi/3];
Zjm={Z1,Z2,Z3} ;


(*%%%%%%%%%%%%%%%%%%% lb=j-1   %%%%%%%%%%%%%%%%%%%%%%%%%%%*)
lb=j-1;
aShaddedMinus=Table[Integrate[Conjugate[Zjm]*SphericalHarmonicY[lb,mb,\[Theta],\[Phi]]*Sin[\[Theta]],{\[Theta],0,Pi},{\[Phi],0,2*Pi}].F[m]*j1*CON*(-I)^(lb+j-1),{mb,lb,-lb,-1}];




lb=j+1;
aShaddedMinus1=Table[Integrate[Conjugate[Zjm]*SphericalHarmonicY[lb,mb,\[Theta],\[Phi]]*Sin[\[Theta]],{\[Theta],0,Pi},{\[Phi],0,2*Pi}].F[m]*CON*j3*(-I)^(lb+j-1),{mb,lb,-lb,-1}];



Print[StringForm["m = ``",-m]];

Print[Simplify[Integrate[r*(aShaddedMinus1.Yjmconj3+aShaddedMinus.Yjmconj1),{\[Phi],0,2*Pi}]]];




]

Print[StringForm["Octopole"]]

j = 3;
(*%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%*)

X1[j_,m_]:=-1/(j*(j+1))^(1/2)*((j*(j+1)-m*(m-1))/2)^(1/2)*SphericalHarmonicY[j,m-1,\[Theta],\[Phi]];
X2[j_,m_]:=1/(j*(j+1))^(1/2)*m*SphericalHarmonicY[j,m,\[Theta],\[Phi]];
X3[j_,m_]:=1/(j*(j+1))^(1/2)*((j*(j+1)-m*(m+1))/2)^(1/2)*SphericalHarmonicY[j,m+1,\[Theta],\[Phi]];
For[nn=0,nn<2j+1,nn++,
m=j-nn;





Xjm={X1[j,m],X2[j,m],X3[j,m]} ;
Xjm//MatrixForm;

Z1= I*I*(-SphericalHarmonicY[1,-1,\[Theta],\[Phi]]*X2[j,m]- SphericalHarmonicY[1,0,\[Theta],\[Phi]]*X1[j,m])*2*Sqrt[Pi/3];
Z2= I*I*(-SphericalHarmonicY[1,-1,\[Theta],\[Phi]]*X3[j,m]+SphericalHarmonicY[1,1,\[Theta],\[Phi]]*X1[j,m])*2*Sqrt[Pi/3];
Z3= I*I*(SphericalHarmonicY[1,0,\[Theta],\[Phi]]*X3[j,m]+SphericalHarmonicY[1,1,\[Theta],\[Phi]]*X2[j,m])*2*Sqrt[Pi/3];
Zjm={Z1,Z2,Z3} ;


(*%%%%%%%%%%%%%%%%%%%%% lb=j-1   %%%%%%%%%%%%%%%%%%%*)
lb=j-1;
aShaddedMinus=Table[Integrate[Conjugate[Zjm]*SphericalHarmonicY[lb,mb,\[Theta],\[Phi]]*Sin[\[Theta]],{\[Theta],0,Pi},{\[Phi],0,2*Pi}].F[m]*j2*CON*(-I)^(lb+j-1),{mb,lb,-lb,-1}];





lb=j+1;
aShaddedMinus1=Table[Integrate[Conjugate[Zjm]*SphericalHarmonicY[lb,mb,\[Theta],\[Phi]]*Sin[\[Theta]],{\[Theta],0,Pi},{\[Phi],0,2*Pi}].F[m]*j4*CON*(-I)^(lb+j-1),{mb,lb,-lb,-1}];



Print[StringForm["m = ``",-m]];

Print[Simplify[Integrate[r*(aShaddedMinus1.Yjmconj4+aShaddedMinus.Yjmconj2),{\[Phi],0,2*Pi}]]]

]

Print[StringForm["4-th order"]]

j = 4;
(*%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%*)

X1[j_,m_]:=-1/(j*(j+1))^(1/2)*((j*(j+1)-m*(m-1))/2)^(1/2)*SphericalHarmonicY[j,m-1,\[Theta],\[Phi]];
X2[j_,m_]:=1/(j*(j+1))^(1/2)*m*SphericalHarmonicY[j,m,\[Theta],\[Phi]];
X3[j_,m_]:=1/(j*(j+1))^(1/2)*((j*(j+1)-m*(m+1))/2)^(1/2)*SphericalHarmonicY[j,m+1,\[Theta],\[Phi]];
For[nn=0,nn<2j+1,nn++,
m=j-nn;





Xjm={X1[j,m],X2[j,m],X3[j,m]} ;
Xjm//MatrixForm;

Z1= I*I*(-SphericalHarmonicY[1,-1,\[Theta],\[Phi]]*X2[j,m]- SphericalHarmonicY[1,0,\[Theta],\[Phi]]*X1[j,m])*2*Sqrt[Pi/3];
Z2= I*I*(-SphericalHarmonicY[1,-1,\[Theta],\[Phi]]*X3[j,m]+SphericalHarmonicY[1,1,\[Theta],\[Phi]]*X1[j,m])*2*Sqrt[Pi/3];
Z3= I*I*(SphericalHarmonicY[1,0,\[Theta],\[Phi]]*X3[j,m]+SphericalHarmonicY[1,1,\[Theta],\[Phi]]*X2[j,m])*2*Sqrt[Pi/3];
Zjm={Z1,Z2,Z3} ;


(*%%%%%%%%%%%%%%%%%%%%%% lb=j-1   %%%%%%%%%%%%%%%%%%%%%%%*)
lb=j-1;
aShaddedMinus=Table[Integrate[Conjugate[Zjm]*SphericalHarmonicY[lb,mb,\[Theta],\[Phi]]*Sin[\[Theta]],{\[Theta],0,Pi},{\[Phi],0,2*Pi}].F[m]*j3*CON*(-I)^(lb+j-1),{mb,lb,-lb,-1}];





lb=j+1;
aShaddedMinus1=Table[Integrate[Conjugate[Zjm]*SphericalHarmonicY[lb,mb,\[Theta],\[Phi]]*Sin[\[Theta]],{\[Theta],0,Pi},{\[Phi],0,2*Pi}].F[m]*j5*CON*(-I)^(lb+j-1),{mb,lb,-lb,-1}];



Print[StringForm["m = ``",-m]];

Print[Simplify[Integrate[r*(aShaddedMinus1.Yjmconj5+aShaddedMinus.Yjmconj3),{\[Phi],0,2*Pi}]]]

]



\end{lstlisting}





\begin{lstlisting}[language=Mathematica,caption={Magnetic multipoles}, numbers=none]
    CON = -k1^2/Sqrt[8 Pi]*1/(Sqrt[(2 Pi)^3]/8/Pi^2);

Yjmconj0 = 1/2/Sqrt[Pi];

conjY11 = 
  Exp[-2*I*\[Phi]]*SphericalHarmonicY[1, 1, \[Theta], \[Phi]];
conjY10 = SphericalHarmonicY[1, 0, \[Theta], \[Phi]];
conjY1m1 = Exp[2*I*\[Phi]]*SphericalHarmonicY[1, -1, \[Theta], \[Phi]];
Yjmconj1 = {conjY11, conjY10, conjY1m1};

conjY2m2 = Exp[4*I*\[Phi]]*SphericalHarmonicY[2, -2, \[Theta], \[Phi]];
conjY2m1 = 
  Exp[2*I*\[Phi]]*SphericalHarmonicY[2, -1, \[Theta], \[Phi]] ;
conjY20 = SphericalHarmonicY[2, 0, \[Theta], \[Phi]];
conjY21 = 
  Exp[-2*I*\[Phi]]*SphericalHarmonicY[2, 1, \[Theta], \[Phi]];
conjY22 = Exp[-4*I*\[Phi]]*SphericalHarmonicY[2, 2, \[Theta], \[Phi]];

Yjmconj2 = {conjY22, conjY21, conjY20, conjY2m1, conjY2m2};

conjY33 = 
  Exp[-6*I*\[Phi]]*SphericalHarmonicY[3, 3, \[Theta], \[Phi]];
conjY32 = 
  Exp[-4*I*\[Phi]]*SphericalHarmonicY[3, 2, \[Theta], \[Phi]];
conjY31 = 
  Exp[-2*I*\[Phi]]*SphericalHarmonicY[3, 1, \[Theta], \[Phi]];
conjY30 = SphericalHarmonicY[3, 0, \[Theta], \[Phi]];
conjY3m1 = Exp[2*I*\[Phi]]*SphericalHarmonicY[3, -1, \[Theta], \[Phi]];
conjY3m2 = Exp[4*I*\[Phi]]*SphericalHarmonicY[3, -2, \[Theta], \[Phi]];
conjY3m3 = Exp[6*I*\[Phi]]*SphericalHarmonicY[3, -3, \[Theta], \[Phi]];

Yjmconj3 = {conjY33, conjY32, conjY31, conjY30, conjY3m1, conjY3m2, 
   conjY3m3};

conjY44 = 
  Exp[-8*I*\[Phi]]*SphericalHarmonicY[4, 4, \[Theta], \[Phi]];
conjY43 = 
  Exp[-6*I*\[Phi]]*SphericalHarmonicY[4, 3, \[Theta], \[Phi]];
conjY42 = 
  Exp[-4*I*\[Phi]]*SphericalHarmonicY[4, 2, \[Theta], \[Phi]];
conjY41 = 
  Exp[-2*I*\[Phi]]*SphericalHarmonicY[4, 1, \[Theta], \[Phi]];
conjY40 = SphericalHarmonicY[4, 0, \[Theta], \[Phi]];
conjY4m1 = Exp[2*I*\[Phi]]*SphericalHarmonicY[4, -1, \[Theta], \[Phi]];
conjY4m2 = Exp[4*I*\[Phi]]*SphericalHarmonicY[4, -2, \[Theta], \[Phi]];
conjY4m3 = Exp[6*I*\[Phi]]*SphericalHarmonicY[4, -3, \[Theta], \[Phi]];
conjY4m4 = Exp[8*I*\[Phi]]*SphericalHarmonicY[4, -4, \[Theta], \[Phi]];

Yjmconj4 = {conjY44, conjY43, conjY42, conjY41, conjY40, conjY4m1, 
   conjY4m2, conjY4m3, conjY4m4} ;

conjY55 = Exp[-10*I*\[Phi]]*SphericalHarmonicY[5, 5, \[Theta], \[Phi]];
conjY54 = 
  Exp[-8*I*\[Phi]]*SphericalHarmonicY[5, 4, \[Theta], \[Phi]];
conjY53 = 
  Exp[-6*I*\[Phi]]*SphericalHarmonicY[5, 3, \[Theta], \[Phi]];
conjY52 = 
  Exp[-4*I*\[Phi]]*SphericalHarmonicY[5, 2, \[Theta], \[Phi]];
conjY51 = 
  Exp[-2*I*\[Phi]]*SphericalHarmonicY[5, 1, \[Theta], \[Phi]];
conjY50 = SphericalHarmonicY[5, 0, \[Theta], \[Phi]];
conjY5m1 = Exp[2*I*\[Phi]]*SphericalHarmonicY[5, -1, \[Theta], \[Phi]];
conjY5m2 = Exp[4*I*\[Phi]]*SphericalHarmonicY[5, -2, \[Theta], \[Phi]];
conjY5m3 = Exp[6*I*\[Phi]]*SphericalHarmonicY[5, -3, \[Theta], \[Phi]];
conjY5m4 = Exp[8*I*\[Phi]]*SphericalHarmonicY[5, -4, \[Theta], \[Phi]];
conjY5m5 = 
  Exp[10*I*\[Phi]]*SphericalHarmonicY[5, -5, \[Theta], \[Phi]];

Yjmconj5 = {conjY55, conjY54, conjY53, conjY52, conjY51, conjY50, 
   conjY5m1, conjY5m2, conjY5m3, conjY5m4, conjY5m5} ;


J1 = (Cos[\[Phi]] - I *Sin[\[Phi]])/Sqrt[2]*(-Jro + I*Jphi);
J0 = Jz;
Jm1 = (Cos[\[Phi]] + I*Sin[\[Phi]])/Sqrt[2]*(Jro + I*Jphi);

F[mb_] := {J1*Exp[I*mb*\[Phi]], J0*Exp[I*mb*\[Phi]], 
   Jm1*Exp[I*mb*\[Phi]]};

Print[StringForm["Dipole"]];
j = 1;
(*%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\
%%%%%%%%%%%%%%%%%%*)

For[nn = 0, nn < 2 j + 1, nn++,
 m = j - nn;
 lb = j;
 X1[j_, m_] := -1/(j*(j + 1))^(1/2)*((j*(j + 1) - m*(m - 1))/2)^(1/2)*
   SphericalHarmonicY[j, m - 1, \[Theta], \[Phi]];
 X2[j_, m_] := 
  1/(j*(j + 1))^(1/2)*m*SphericalHarmonicY[j, m, \[Theta], \[Phi]];
 X3[j_, m_] := 
  1/(j*(j + 1))^(1/2)*((j*(j + 1) - m*(m + 1))/2)^(1/2)*
   SphericalHarmonicY[j, m + 1, \[Theta], \[Phi]];
 
 Xjm = {X1[j, m], X2[j, m], X3[j, m]} ;
 Xjm // MatrixForm;
 
 bShadded = 
  Table[Integrate[
      Conjugate[Xjm]*SphericalHarmonicY[lb, mb, \[Theta], \[Phi]]*
       Sin[\[Theta]], {\[Theta], 0, Pi}, {\[Phi], 0, 2*Pi}] . F[m]*j1*
    CON *(-I)^(2*j), {mb, j, -j, -1}];
 Print[StringForm["m= ``", -m]];
 
 Print[Simplify[Integrate[r*bShadded . Yjmconj1, {\[Phi], 0, 2*Pi}]]]
 ]


Print[StringForm["Quadropole"]];

j = 2;
(*%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\
%%%%%%%%%%%%%%%%%%*)

For[nn = 0, nn < 2 j + 1, nn++,
 m = j - nn;
 lb = j;
 X1[j_, m_] := -1/(j*(j + 1))^(1/2)*((j*(j + 1) - m*(m - 1))/2)^(1/2)*
   SphericalHarmonicY[j, m - 1, \[Theta], \[Phi]];
 X2[j_, m_] := 
  1/(j*(j + 1))^(1/2)*m*SphericalHarmonicY[j, m, \[Theta], \[Phi]];
 X3[j_, m_] := 
  1/(j*(j + 1))^(1/2)*((j*(j + 1) - m*(m + 1))/2)^(1/2)*
   SphericalHarmonicY[j, m + 1, \[Theta], \[Phi]];
 
 Xjm = {X1[j, m], X2[j, m], X3[j, m]} ;
 Xjm // MatrixForm;
 
 bShadded = 
  Table[Integrate[
      Conjugate[Xjm]*SphericalHarmonicY[lb, mb, \[Theta], \[Phi]]*
       Sin[\[Theta]], {\[Theta], 0, Pi}, {\[Phi], 0, 2*Pi}] . F[m]*j2*
    CON *(-I)^(2*j), {mb, j, -j, -1}];
 
 Print[StringForm["m= ``", -m]];
 Print[Simplify[
   Integrate[r*bShadded . Yjmconj2, {\[Phi], 0, 2*Pi}]]];
 ]



Print[StringForm["Octopole"]];

j = 3;
(*%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\
%%%%%%%%%%%%%%%%%%*)

For[nn = 0, nn < 2 j + 1, nn++,
 m = j - nn;
 lb = j;
 X1[j_, m_] := -1/(j*(j + 1))^(1/2)*((j*(j + 1) - m*(m - 1))/2)^(1/2)*
   SphericalHarmonicY[j, m - 1, \[Theta], \[Phi]];
 X2[j_, m_] := 
  1/(j*(j + 1))^(1/2)*m*SphericalHarmonicY[j, m, \[Theta], \[Phi]];
 X3[j_, m_] := 
  1/(j*(j + 1))^(1/2)*((j*(j + 1) - m*(m + 1))/2)^(1/2)*
   SphericalHarmonicY[j, m + 1, \[Theta], \[Phi]];
 
 Xjm = {X1[j, m], X2[j, m], X3[j, m]} ;
 Xjm // MatrixForm;
 
 bShadded = 
  Table[Integrate[
      Conjugate[Xjm]*SphericalHarmonicY[lb, mb, \[Theta], \[Phi]]*
       Sin[\[Theta]], {\[Theta], 0, Pi}, {\[Phi], 0, 2*Pi}] . F[m]*j3*
    CON *(-I)^(2*j), {mb, j, -j, -1}];
 
 Print[StringForm["m= ``", -m]];
 Print[Simplify[Integrate[r*bShadded . Yjmconj3, {\[Phi], 0, 2*Pi}]]]
 ]

Print[StringForm["4-th order"]];

j = 4;
(*%%%%%%%%%%%%%%%%%%%%%%%%%\
%%%%%%%%%%%%%%%%%%*)

For[nn = 0, nn < 2 j + 1, nn++,
 m = j - nn;
 lb = j;
 X1[j_, m_] := -1/(j*(j + 1))^(1/2)*((j*(j + 1) - m*(m - 1))/2)^(1/2)*
   SphericalHarmonicY[j, m - 1, \[Theta], \[Phi]];
 X2[j_, m_] := 
  1/(j*(j + 1))^(1/2)*m*SphericalHarmonicY[j, m, \[Theta], \[Phi]];
 X3[j_, m_] := 
  1/(j*(j + 1))^(1/2)*((j*(j + 1) - m*(m + 1))/2)^(1/2)*
   SphericalHarmonicY[j, m + 1, \[Theta], \[Phi]];
 
 Xjm = {X1[j, m], X2[j, m], X3[j, m]} ;
 Xjm // MatrixForm;
 
 bShadded = 
  Table[Integrate[
      Conjugate[Xjm]*SphericalHarmonicY[lb, mb, \[Theta], \[Phi]]*
       Sin[\[Theta]], {\[Theta], 0, Pi}, {\[Phi], 0, 2*Pi}] . F[m]*j4*
    CON *(-I)^(2*j), {mb, j, -j, -1}];
 
 Print[StringForm["m= ``", -m]];
 Print[Simplify[Integrate[r*bShadded . Yjmconj4, {\[Phi], 0, 2*Pi}]]]
 ]

\end{lstlisting}

==> sections/scs_acs_ecs.tex <==
\subsection{Scattering cross-section}
The Poynting vector for the scattered field corresponding the angular harmonic $e^{-im\varphi}$ can be written as 
\begin{equation}\label{eq:9}
    \vb S_m^\text{scat} = \dfrac 12 \text{Re}[\vb E_m^\text{scat} \times\vb H_m^\text{scat*}], 
\end{equation}
Thus, the partial scattering cross-section is 
 \begin{equation}
 \begin{aligned}
    \sigma_m^\text{scat} = & \frac{1}{I_{\text{inc}}}\int_{S^2} (\vb S_m^\text{scat}\cdot \vb n)\ \dd s = \\ = &
    \frac{1}{I_{\text{inc}}}\int_{C_R} 2\pi \rho (\vb S_m^\text{scat}\cdot \vb n)\ \dd c,
\end{aligned}
\end{equation}
where $I_{\text{inc}}= |E^{\text{inc}}|^2/(2Z)$ is the energy flux of the incident wave,  $Z = \sqrt{{\mu_0}/{\varepsilon_0}}$ is the impedance of the embedding medium (vacuum in our case), and  the integral is taken over the sphere $S^2$ surrounding the structure. 
In 2D axial symmetry this sphere become semi-circle $C_R$ (see Fig.~\ref{fig:concept}).
For 2D geometry integral over the angle $\varphi$ gives the multiplier 
$2\pi\rho$, and  $\dd c$ is the circle arc length differential.
We note that COMSOL\textsuperscript{\textregistered} allows omission of the $2\pi\rho$ multiplier if the \texttt{Compute surface integral} option is selected.
See details of the derivation in the Supplemental Material.

Due to orthogonality of the electromagnetic modes with different $m$, the total scattering cross-section can be obtained by summing over all orders $m$: 
 \begin{equation}\label{eq:10}
    \sigma^{\text{scat}}=\sum_{m = 0}^{\infty} (2-\delta_{0,m}) \sigma_m^\text{scat} ,
 \end{equation}
where $\delta_{0,m}$ is the Kronecker symbol, which appears due to $\sigma_m^\text{scat} = \sigma_{-m}^\text{scat}$, according to the properties of the problem {[see Eq.~\eqref{eq:even-odd}]}.

\subsection{Absorption cross-section}

As well as scattering cross-section, the total absorption cross-section $\sigma^\text{abs}$ can be calculated as a sum of partial absorption cross-sections $\sigma^\text{abs}_m$:
\begin{equation}
\label{eq:t_abs_CS}
    \sigma^\text{abs} = \sum_{m = 0}^{\infty}
    (2 - \delta_{0,m})\sigma^\text{abs}_m.
\end{equation}
Each partial absorption cross-section can be calculated through the following volume integral:
\begin{equation}
\label{eq:p_abs_CS}
    \sigma^\text{abs}_m=\frac{\omega\pi}{I_\text{inc}}\iint_\Omega
    \text{Im}\left\{\mathbf{P}_m^*\mathbf{E}_m\right\} \rho \mathrm{d}\rho\mathrm{d}z.
\end{equation}
Here, $\mathbf{P}_m=\varepsilon_0(\varepsilon-1)\mathbf{E}_m$ is the polarization, $\varepsilon$ is the dielectric permittivity of the scatterer's material.
The integral is taken over the cross-section area $\Omega$ of the scatterer [see Fig.~\ref{fig:concept}(a)].
See details of the derivation in the Supplemental Material.

\subsection{Extinction cross-section}

The total extinction cross-section $\sigma^\text{ext}$ can be calculated as the sum of the partial extinction cross-sections $\sigma^\text{ext}_m$ corresponding to different $m$ by analogy with Eqs.~\eqref{eq:10} and \eqref{eq:t_abs_CS}.
The partial extinction cross-sections can be calculated in several ways:
\begin{itemize}
    \item[(i)] By definition of the extinction cross-section:
    \begin{equation}
        \sigma^\text{ext}_m=\sigma^\text{scat}_m+\sigma^\text{abs}_m.
    \end{equation}
    \item[(ii)] By taking a surface integral over the cross-section area $\Omega$ of the scatterer [see Fig.~\ref{fig:concept}(a)]:
    \begin{equation}
    \label{eq:p_ext_CS}
        \sigma^\text{ext}_m=\frac{\omega\pi}{I_\text{inc}}\iint_\Omega
        \text{Im}\left\{\mathbf{P}_m^*\mathbf{E}^\text{inc}_m\right\} \rho \mathrm{d}\rho\mathrm{d}z.
    \end{equation}
    \item[(iii)] {By taking a line integral over $C_R$ [see Fig.~\ref{fig:concept}(a)]:
    \begin{equation}
        \sigma_m^\text{ext} = \frac{1}{I_{\text{inc}}}\int_{C_R} 2\pi  \rho (\vb S_m^\text{ext}\cdot \vb n)\ \dd c,
    \end{equation}
    where
    \begin{equation}
        \vb S_m^\text{ext}=-\frac{1}{2}\text{Re}
        \left\{
        \mathbf{E}_m^\text{inc}\times\mathbf{H}_m^{\text{scat}*}+
        \mathbf{E}_m^\text{scat}\times\mathbf{H}_m^{\text{inc}*}
        \right\}.    
    \end{equation}}
\end{itemize}
Therefore, scattering, absorption and extinction cross sections of an axially symmetric scatterer can be calculated using both surface or line integral.
See details of the derivation in the Supplemental Material.


\subsection{Maxwell stress tensor and optical forces}

Optical force is widely studied in nanooptics and nanophotonics as it allows for trapping and manipulating micro- and  nanoobjects via optical fields~\cite{Ashkin1997May,Marago2013Nov,Ivinskaya2017May}.    While the optical force can be directly computed by integrating the Maxwell stress-tensor over the area containing the scatterer, one still needs to know the electromagnetic fields distribution in the near- or far-zones.
One can connect the terms with different $m$ and optical forces in order to effectively compute the forces acting on a scatterer with rotational symmetry.
Indeed, the Maxwell stress-tensor has the form \cite{Novotny2012Sep}
\begin{equation}
\label{eq:Max_st_tens}
    \widehat{T} = \varepsilon_{0}\mathbf{E} \otimes \mathbf{E} + \mu_{0}\mathbf{H} \otimes \mathbf{H} - \frac{1}{2}\left( \varepsilon_{0}\mathbf{E}\mathbf{E} + \mu_{0}\mathbf{H}\mathbf{H} \right)\widehat{I}.
\end{equation}
Here $\varepsilon_{0}$ and $\mu_{0}$ are the permittivity and permeability of vacuum, $\widehat{I}$ is the identity tensor.
The optical force can be calculated by integration of Eq.~\eqref{eq:Max_st_tens} over the closed area containing the scatterer: 
\begin{align}
\label{eq:force}
    \vb F=\oint_{S^2}\widehat{T} \mathrm{d}s. 
\end{align}
Substituting expansion~\eqref{eq:cyl_decomp} into Eq.~\eqref{eq:force} one can reduce the integration to the integration over the line $C_R$ and summation over the harmonics.
The $x$-component of the force acting on the scatterer has the following form
 \begin{equation}
     \left\langle F_x\right\rangle = \left\langle F^\text{E}_x\right\rangle + \left\langle F^\text{H}_x\right\rangle,
 \end{equation}
where
\begin{equation}
\begin{aligned}
    \left\langle {F}^\text{E}_{x}\right\rangle 
    & = \frac{\varepsilon_0}{4}\mathop{\mathrm{Re}}\int_{C_R}^{}{2\pi {\rho}\, \mathrm{d}c}\,\sum_{m = - \infty}^{ \infty}\left\lbrack \left( E_{m,\rho}\left( E_{m + 1,\rho} \right)^{*} - \right.  \right.  \\ 
    & -  \left. \left. E_{m,\varphi}\left( E_{m + 1,\varphi} \right)^{*} - E_{m,z}\left( E_{m + 1,z} \right)^{*} -\right.\right.\\
     & - \left. \left. iE_{m,\rho}\left( E_{m + 1,\varphi} \right)^{*} + iE_{m + 1,\rho}\left( E_{m,\varphi} \right)^{*} \right)n_{\rho}+\right.  \\
     & + \left. 2E_{m,\rho}\left( E_{m,z} \right)^{*}n_{z} \right \rbrack.
\end{aligned}
\end{equation}
Here $n_{\rho}$ and $n_z$ are the coordinate-dependent components of the vector normal to the integration surface,  and $\left\langle F^\text{H}_x\right\rangle$ satisfies the same equation after replacing $\varepsilon_0$ with $\mu_0$ and $\vb E$ with $\vb H$.
We refer readers to the Supplementary Materials, where they can find details on the derivation of the formulas above and the expressions for other components of the optical force.
